ScooterLab: A Programmable and Participatory Sensing Research Testbed using Micromobility Vehicles

Micromobility vehicles, such as e-scooters, are increasingly popular in urban communities but present significant challenges in terms of road safety, user privacy, infrastructure planning, and civil engineering. Addressing these critical issues requires a large-scale and easily accessible research infrastructure to collect diverse mobility and contextual data from micromobility users in realistic settings. To this end, we present ScooterLab, a community research testbed comprising a fleet of customizable battery-powered micromobility vehicles retrofitted with advanced sensing, communication, and control capabilities. ScooterLab enables interdisciplinary research at the intersection of computing, mobility, and urban planning by providing researchers with tools to design and deploy customized sensing experiments and access curated datasets. The testbed will enable advances in machine learning, privacy, and urban transportation research while promoting sustainable mobility.

==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

ScooterLab establishes a flexible platform for micromobility research, enabling data-driven studies across safety, infrastructure, and environmental domains. Through its unique setup and accessible data resources, it offers a practical approach to advancing knowledge in urban and transportation studies, benefiting researchers and city planners alike.



